PVP: Polar Representation Boost for 3D Semantic Occupancy Prediction

Recently, polar coordinate-based representations have shown promise for 3D perceptual tasks. Compared to Cartesian methods, polar grids provide a viable alternative, offering better detail preservation in nearby spaces while covering larger areas. However, they face feature distortion due to non-uniform division. To address these issues, we introduce the Polar Voxel Occupancy Predictor (PVP), a novel 3D multi-modal predictor that operates in polar coordinates. PVP features two key design elements to overcome distortion: a Global Represent Propagation (GRP) module that integrates global spatial data into 3D volumes, and a Plane Decomposed Convolution (PD-Conv) that simplifies 3D distortions into 2D convolutions. These innovations enable PVP to outperform existing methods, achieving significant improvements in mIoU and IoU metrics on the OpenOccupancy dataset.

==> text/tmp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Your abstract is well-structured and conveys the main ideas effectively. However, I noticed a few grammatical and stylistic improvements that can be made. Here's a revised version:

---

Recently, polar-based representations have demonstrated promising attributes in perceptual tasks. In contrast to Cartesian-based approaches, representing surrounding spaces using polar grids is now recognized as a viable alternative, thanks to its aptitude for representing vast spaces and retaining intricate details of proximate areas. Nevertheless, when addressing the newly introduced dense voxel segmentation—where the objective is to predict the semantic occupancy of each voxel within the designated 3D space—polar-based methods grapple with the feature distortion issue. This arises from the non-uniform division inherent to polar representation, thereby curtailing the efficacy of these polar techniques. 

To address this challenge, we introduce PVP, a straightforward yet potent 3D occupancy predictor utilizing polar coordinates. PVP mitigates the feature distortion quandary through two distinct mechanisms: 1) a global representation propagation module that infuses global spatial data into the intermediate 3D volume, factoring in the spatial structure precedence, and 2) a plane-decomposed convolution that segments the original 3D spatial convolution into multiple 2D convolutions, each operating on a separate plane. 

Thanks to these pragmatic alterations, our method eclipses preceding works by significant margins: 1.9% mIoU and 2.9% IoU when compared to Lidar-only techniques, and 7.5% mIoU and 6.1% IoU against multimodal methods on the OpenOccupancy validation set. Consequently, our approach delivers results that stand shoulder-to-shoulder with the state-of-the-art methodologies.

---

Some key changes I made:

1. Changed some word choices to improve clarity and readability.
2. Broke down longer sentences to enhance comprehension.
3. Fixed minor grammatical errors and redundancies. 

Feel free to adjust further based on your preferences and technical accuracy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% abs shorter
In recent developments, polar-based representations have emerged as a promising alternative to Cartesian-based approaches for perceptual tasks. These representations excel in capturing expansive spaces while maintaining intricate details of proximate regions. However, in the context of the burgeoning area of dense voxel segmentation—aimed at determining the semantic occupancy of every voxel within a specified 3D space—polar-based methodologies exhibit significant shortcomings due to the inherent feature distortion arising from their non-uniform division. In this paper, we introduce PVMO, an innovative 3D occupancy predictor leveraging polar coordinates. PVMO adeptly addresses feature distortion through two pivotal mechanisms: 1) global decomposed re-alignment, which infuses global spatial information into the intermediary 3D volume, and 2) spatial decomposed convolution, which parses the standard 3D spatial convolution into multiple 2D convolutions across individual planes. Through these nuanced yet impactful modifications, PVMO surpasses preceding models by achieving a notable 7.5% mIoU and 6.1% IoU improvement on the OpenOccupancy validation dataset, positioning it competitively against contemporary state-of-the-art techniques.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% introduction
In autonomous driving systems, the accurate perception of 3D structural information, encompassing both objects and regions, becomes paramount, especially in the absence of HD maps. Historically, tasks like 3D object detection and 3D semantic segmentation have primarily concentrated on foreground objects or scanned points. These efforts often neglect a detailed representation of the surrounding environment and exhibit limited generalization to objects with unfamiliar geometries. Given these challenges, the field has increasingly pivoted towards 3D occupancy prediction, which seeks to assign a semantic label to every voxel within the perceptual range, thus making it a cornerstone for 3D scene comprehension in autonomous driving.

Pioneering methods, as detailed in~\cite{huang2023tri, zhang2023occformer, wang2023openoccupancy, wei2023surroundocc}, have harnessed an array of techniques to yield appropriate feature representations for each voxel. Notably, TPVFormer~\cite{huang2023tri} innovatively models space using a tri-plane paradigm and employs sparse sampling for voxel prediction supervision, underscoring the potential of 2D representation. Meanwhile, SurroundOcc~\cite{wei2023surroundocc} adopts the BEVFormer's~\cite{li2022bevformer} framework, and OccFormer~\cite{zhang2023occformer} alongside CONet~\cite{wang2023openoccupancy} employ the lift-splat-shoot strategy for spatial volume feature generation, each introducing distinct features to augment performance.

However, a predominant reliance on Cartesian-based volumetric representation confronts these methods. Such representation engenders issues stemming from uniform voxel distribution across distances, causing computational inefficiencies and information paucity, especially for distal regions. The polar representation emerges as a solution, with its volume modulating with distance to adeptly correspond with the uneven distribution of geometric and semantic information inherent to point clouds and camera feeds. The successes of the polar representation in tasks like LiDAR semantic segmentation~\cite{zhang2020polarnet, zhu2021cylindrical} and 3D object detection~\cite{nie2023partner} further embolden its application in 3D occupancy prediction. Nevertheless, its adoption is not without complications. As delineated in Fig.~\ref{fig-distort}, polar grids introduce distortions that manifest as two primary challenges in representation.

In response to these challenges, this paper introduces the \textbf{P}olar \textbf{V}oxel \textbf{Multi}-modality \textbf{O}ccupancy Predictor (PVMO), a novel model devised to effectively harness polar coordinates. At its core, PVMO incorporates two integral components: the Global Representation Propagation Module (GRP Module) and the Spatial Plane Decomposed Convolution (SPD-Conv). The former employs a unique attention mechanism to discern and propagate road structures, while the latter addresses local distortion through a nuanced convolutional approach. Empirically, our model consistently surpasses extant methodologies.

In summary, our contributions are three-fold:
\textbf{(i)} We delve into the intricacies of feature distortion in polar volume representation and proffer PVMO, a groundbreaking 3D occupancy predictor.
\textbf{(ii)} We present two bespoke designs catered to the polar domain, emphasizing global representation realignment and geometry-informed prediction.
\textbf{(iii)} Comprehensive evaluations on the OpenOccupancy highlight PVMO's stellar performance metrics, revealing its efficacy with both LiDAR and multimodal inputs, and outstripping contemporary models.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% INTRO 2ND VERSION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the realm of autonomous driving systems, the accurate perception of 3D structural information pertaining to surrounding scenes, inclusive of both objects and regions, assumes critical significance, particularly in the absence of HD maps. Traditional tasks, such as 3D object detection and 3D semantic segmentation, predominantly concentrate on foreground objects or scanned points. Such a narrowed focus impedes the generation of comprehensive shape details of the ambient environment and hampers generalization across objects with unobserved contours. Addressing these constraints, there has been a notable shift towards 3D occupancy prediction, which endeavors to attribute a semantic label to every voxel within the perceptual range. This approach is steadily establishing itself as an integral component of 3D scene comprehension in autonomous driving.

A review of the literature reveals varied methodologies designed to derive pertinent representative features for each voxel. For instance, TPVFormer~\cite{huang2023tri} employs a tri-plane approach to model surrounding space, harnessing sparse sampling to guide the voxel prediction head. This sheds light on the prospective advantages of 2D representation coupled with sampling-based supervision. On a parallel trajectory, SurroundOcc~\cite{wei2023surroundocc} extrapolates the framework of BEVFormer~\cite{li2022bevformer}, utilizing a consortium of spatial queries and multi-scale feature aggregation to derive the spatial volume feature. Subsequent feature extraction is performed using a 3D convolution network. Further, both OccFormer~\cite{zhang2023occformer} and CONet~\cite{wang2023openoccupancy} adopt the lift-splat-shoot pipeline for the generation of spatial volume features. Notably, OccFormer augments this with additional BEV features and introduces a window-attention-based FPN fortified with cross-attention to leverage these supplementary BEV features. Pioneering a novel approach, CONet stands out as the inaugural model to inaugurate a contemporary multi-modality pipeline, furthering the technique with direct sampling for predictions from a 4x down-sampled volume.

However, a salient observation underscores that the prevailing methodologies predominantly lean on Cartesian-based volumetric representations. Such methods grapple with the challenge of maintaining a uniform voxel distribution across varying distances. Given that distant terrains possess equivalent voxel density as proximal areas, there exists a palpable disparity. The tangible data, such as point clouds or visual cues from imagery pertinent to distant regions, is inherently sparse, attributed to sensor limitations. This culminates in computational inefficiencies and a pronounced dearth of voxel-specific information.


The potential of polar representation in addressing the issues of uniform voxel distribution is becoming increasingly evident. This representation, with its volume variations in accordance with distance, aptly resonates with the disparate distribution of geometric information derived from point clouds and semantic data from cameras. Its successful application in tasks like LiDAR semantic segmentation~\cite{zhang2020polarnet, zhu2021cylindrical} and 3D object detection~\cite{nie2023partner} further propels our interest to harness polar representation for 3D occupancy prediction. Nonetheless, while promising, polar-based 3D occupancy predictors are not exempt from challenges, most notably, feature distortions.

As depicted in Fig.~\ref{fig-distort}, polar grid representations yield distorted renditions of scenes based on range. This distortion is the precursor to two primary impediments. Firstly, the pronounced variations in local structure occupancy within polar grids render translation-invariant convolutions incompatible with non-rectangular structures. This incongruence gives rise to maladaptive local features, thereby undermining the efficacy of polar-based predictors. Additionally, as emphasized by Fig.~\ref{fig-distort}, elements such as roads, sidewalks, and ground surfaces exhibit profound distortions in their overarching structure. Consequently, transitioning from sparse feature grids to dense features becomes problematic, as localized feature propagation techniques, be it convolution or window attention, struggle to discern the holistic structure of these entities, impairing accurate feature propagation.

Earlier attempts to navigate this conundrum include PolarStream's~\cite{chen2021polarstream} range-stratified convolutions. However, its intricate design could not seamlessly align features for efficient object recognition. PARTNER~\cite{nie2023partner} initiated mechanisms for foreground object feature alignment, but this was somewhat myopic, solely focusing on foreground objects and overlooking the broader feature propagation challenges.

In response, we introduce the \textbf{P}olar \textbf{V}oxel \textbf{Multi}-modality \textbf{O}ccupancy Predictor (PVMO), a streamlined yet potent solution designed to optimize representation in polar coordinates. Our model pivots on two primary innovations: the Global Representation Propagation Module (GRP Module) and the Spatial Plane Decomposed Convolution (SPD-Conv). The GRP Module leverages a unique attention mechanism to discern road structures from scene volumes, facilitating precise feature propagation. To ensure computational efficiency, prior to global attention, the input volume undergoes window attention, which refines the feature set. Post this refinement, dimension-wise self-attention is engaged for holistic feature propagation. Addressing local distortions inherent to polar volumes, the spatial decomposed convolution is introduced. By supplanting 3D convolution with a trio of 2D convolutions, intricate 3D distortions are distilled into a series of transformations across different planes. With these enhancements, PVMO redefines excellence, outclassing existing solutions in polar 3D occupancy prediction.

To encapsulate, our salient contributions are:
\textbf{(i)} A meticulous exploration of feature distortion in polar volume representation, leading to the conceptualization of a pioneering 3D occupancy predictor, PVMO, rooted in the polar coordinate system.
\textbf{(ii)} The debut of two polar-specific innovations: a global representation propagation module to recalibrate distorted polar features and a geometry-aware adaptive head to hone box prediction accuracy.
\textbf{(iii)} Comprehensive validation of our innovations on the OpenOccupancy dataset, wherein PVMO exhibits significant advancements over benchmark methods across both geometric and semantic evaluations, asserting its superiority for both LiDAR and multi-modal inputs.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%% INTRO 2nd version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
In the realm of autonomous driving systems, the accurate perception of 3D structural information pertaining to surrounding scenes, inclusive of both objects and regions, assumes critical significance, particularly in the absence of HD maps. 

Traditional tasks, such as 3D object detection and 3D semantic segmentation, predominantly concentrate on foreground objects or scanned points. Such a narrowed focus impedes the generation of comprehensive shape details of the ambient environment and hampers generalization across objects with unobserved contours. Addressing these constraints, there has been a notable shift towards 3D occupancy prediction, which endeavors to attribute a semantic label to every voxel within the perceptual range. This approach is steadily establishing itself as an integral component of 3D scene comprehension in autonomous driving.

A review of the literature reveals varied methodologies designed to derive pertinent representative features for each voxel. For instance, TPVFormer~\cite{huang2023tri} employs a tri-plane approach to model surrounding space, harnessing sparse sampling to guide the voxel prediction head. This sheds light on the prospective advantages of 2D representation coupled with sampling-based supervision. On a parallel trajectory, SurroundOcc~\cite{wei2023surroundocc} extrapolates the framework of BEVFormer~\cite{li2022bevformer}, utilizing a consortium of spatial queries and multi-scale feature aggregation to derive the spatial volume feature. Subsequent feature extraction is performed using a 3D convolution network. Further, both OccFormer~\cite{zhang2023occformer} and CONet~\cite{wang2023openoccupancy} adopt the lift-splat-shoot pipeline for the generation of spatial volume features. Notably, OccFormer augments this with additional BEV features and introduces a window-attention-based FPN fortified with cross-attention to leverage these supplementary BEV features. Pioneering a novel approach, CONet stands out as the inaugural model to inaugurate a contemporary multi-modality pipeline, furthering the technique with direct sampling for predictions from a 4x down-sampled volume.

However, a salient observation underscores that the prevailing methodologies predominantly lean on Cartesian-based volumetric representations. Such methods grapple with the challenge of maintaining a uniform voxel distribution across varying distances. Given that distant terrains possess equivalent voxel density as proximal areas, there exists a palpable disparity. The tangible data, such as point clouds or visual cues from imagery pertinent to distant regions, is inherently sparse, attributed to sensor limitations. This culminates in computational inefficiencies and a pronounced dearth of voxel-specific information.

In the context of 3D representation for autonomous systems, the polar paradigm has demonstrated its potential to address the inherent challenges of uniform voxel distribution. The polar model's volumetric variation with distance inherently aligns with the asymmetric distribution of geometric data from point clouds and semantic insights from cameras. The polar representation's evident efficacy in tasks such as LiDAR semantic segmentation~\cite{zhang2020polarnet, zhu2021cylindrical} and 3D object detection~\cite{nie2023partner} further motivates our exploration of its applicability to 3D occupancy prediction. 

Nevertheless, while polar representation holds promise, it is not without its challenges. A crucial hurdle is its predisposition to feature distortion. As depicted in Fig.~\ref{fig-distort}, classes such as roads, sidewalks, and ground surfaces undergo pronounced structural distortions. This complicates the process of propagating features from sparse grids to denser counterparts, as conventional tools like convolution or window attention potentially fall short in comprehending the global structures and directing features to the corresponding voxels. Prior work, like PolarStream~\cite{chen2021polarstream}, endeavored to navigate these challenges using range-stratified convolutions, yet their design could not consistently realign features for effective object discernment. Another attempt, PARTNER~\cite{nie2023partner}, took strides in realigning foreground object features, but its scope remained confined to these objects, not addressing the broader propagation issue.

In response to these challenges, we unveil the \textbf{P}olar \textbf{V}oxel \textbf{Multi}-modality \textbf{O}ccupancy Predictor, abbreviated as PVMO, tailored for efficient polar coordinate representation. Central to our approach are two pivotal components: the Global Representation Propagation Module (GRP Module) and the Spatial Plane Decomposed Convolution (SPD-Conv). The GRP Module harnesses an avant-garde attention mechanism to glean road structure from the scene volume, ensuring accurate feature propagation. To preclude the necessity for expansive global attention, we first refine the input volume using window attention to capture the salient features. This is followed by a dimension-wise self-attention for holistic feature propagation. To address local distortion, we introduce the spatial decomposed convolution, in tune with polar volume properties. Transitioning from 3D to three individual 2D convolutions allows the intricate 3D distortions to be resolved into a range plane scale transformation, a BEV plane projection transformation, and a slicing plane identity transformation. Equipped with our tailored designs, PVMO stands out, eclipsing existing methods in 3D occupancy prediction.

To encapsulate, our primary contributions include:
\textbf{(i)} A detailed exploration of the feature distortion challenge intrinsic to polar volume representation, leading to the introduction of a groundbreaking 3D occupancy predictor—PVMO—within the polar coordinate framework.
\textbf{(ii)} The innovation of two polar-centric designs: a global representation realignment module that rectifies feature distortions inherent to polar bases, and a geometry-attuned adaptive head ensuring precise box forecasting.
\textbf{(iii)} A comprehensive validation of our designs' efficacy on the OpenOccupancy dataset. Significantly, PVMO achieves unmatched performance improvements against benchmarked methods, showcasing unparalleled prowess for both LiDAR and multi-modal inputs.

==> text/tmp0930.tex <==
%%%%%%%%%% abs 
Your abstract is well-structured and conveys the main ideas effectively. However, I noticed a few grammatical and stylistic improvements that can be made. Here's a revised version:

---

Recently, polar-based representations have demonstrated promising attributes in perceptual tasks. In contrast to Cartesian-based approaches, representing surrounding spaces using polar grids is now recognized as a viable alternative, thanks to its aptitude for representing vast spaces and retaining intricate details of proximate areas. Nevertheless, when addressing the newly introduced dense voxel segmentation—where the objective is to predict the semantic occupancy of each voxel within the designated 3D space—polar-based methods grapple with the feature distortion issue. This arises from the non-uniform division inherent to polar representation, thereby curtailing the efficacy of these polar techniques. 

To address this challenge, we introduce PVP, a straightforward yet potent 3D occupancy predictor utilizing polar coordinates. PVP mitigates the feature distortion quandary through two distinct mechanisms: 1) a global representation propagation module that infuses global spatial data into the intermediate 3D volume, factoring in the spatial structure precedence, and 2) a plane-decomposed convolution that segments the original 3D spatial convolution into multiple 2D convolutions, each operating on a separate plane. 

Thanks to these pragmatic alterations, our method eclipses preceding works by significant margins: 1.9% mIoU and 2.9% IoU when compared to Lidar-only techniques, and 7.5% mIoU and 6.1% IoU against multimodal methods on the OpenOccupancy validation set. Consequently, our approach delivers results that stand shoulder-to-shoulder with the state-of-the-art methodologies.

---

Some key changes I made:

1. Changed some word choices to improve clarity and readability.
2. Broke down longer sentences to enhance comprehension.
3. Fixed minor grammatical errors and redundancies. 

Feel free to adjust further based on your preferences and technical accuracy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Your introduction is detailed and conveys complex ideas related to 3D occupancy prediction and autonomous driving systems. I have made some revisions for clarity, grammar, and coherence. Here's your revised introduction:

---

In the realm of autonomous driving systems, accurately perceiving the 3D structural information of surrounding scenes—including both objects and regions—is of paramount importance, especially in the absence of HD maps. Historically, tasks such as 3D object detection and 3D semantic segmentation have focused predominantly on foreground objects or scanned points. This narrow focus restricts the generation of a holistic understanding of the environment's shape details and hinders generalization across objects with unfamiliar shapes.

To counter these limitations, there has been a noticeable shift towards 3D occupancy prediction, which aims to assign a semantic label to each voxel within the perceptual range. This approach has garnered increasing attention and has begun to serve as a vital component for 3D scene understanding in autonomous driving.

Previous methods, as cited by [1-4], have delved into diverse techniques to derive representative features for each voxel. TPVFormer [1] innovatively models the surrounding space tri-planarly and employs sparse sampling to guide the voxel prediction head, highlighting the potential of 2D representation and sampling-based supervision. SurroundOcc [4] builds on BEVFormer's [5] methodology, using spatial queries and multi-scale feature aggregation to extract the spatial volume feature before employing a 3D convolution network for final feature derivation. Both OccFormer [2] and CONet [3] utilize the lift-splat-shoot pipeline to generate spatial volume features, with OccFormer incorporating additional BEV features through a window-attention-based FPN with cross-attention. Meanwhile, CONet pioneers a contemporary multi-modality pipeline with direct sampling to draw the final prediction from a 4x down-sampled volume.

However, many popular methods rely on Cartesian-based volumetric representation, leading to the challenge of uniform voxel distribution over varying distances. The equal voxel density between distant and proximate regions results in computational inefficiencies and insufficient information in each voxel due to sensor limitations. Polar representation offers a potential solution, as its volume adjusts with distance, harmonizing with the unbalanced distribution of geometric information from point clouds and semantic data from cameras. Its success in tasks such as LiDAR semantic segmentation [6-7] and 3D object detection [8] propels us to consider polar representation for 3D occupancy prediction. Yet, polar-based 3D occupancy predictors face pronounced feature distortions, as scenes depicted by polar grids appear distorted by range [8]. This distortion manifests two primary challenges: the misalignment of local structures on polar grids with translation-invariant convolution, leading to suboptimal local features, and the significant distortion of entities like roads or sidewalks, making feature propagation from sparse grids challenging. While attempts like PolarStream [9] and PARTNER [8] have been made to tackle these issues, they offer partial solutions, emphasizing only certain aspects or objects.

To rectify the aforementioned challenges, we unveil the **Polar Voxel Occupancy Predictor (PVP)**, a straightforward yet efficacious tool for learning representations in polar coordinates. Our approach features two primary components: the global representation propagation module (GRP Module) and the plane decomposed convolution (PD-Conv). The GRP Module employs a unique attention mechanism to discern road structures from scene volumes and accurately propagate features. We initiate this by condensing the input volume using window attention. Following this, dimension-wise self-attention is executed for global feature propagation. To address local distortions inherent in polar volumes, we introduce a spatial decomposed convolution. By supplanting the 3D convolution with three 2D convolutions, intricate 3D distortions are parsed into a range of transformations across different planes. Armed with these innovations, our polar 3D Occupancy Predictor surpasses all existing methodologies.

In summary, our contributions are:
**i)** Exploration of the feature distortion challenge in polar volume representation, leading to the inception of a pioneering 3D occupancy predictor, PVP, rooted in the polar coordinate system.
**ii)** Introduction of two polar-centric designs: a global representation propagation module for optimal feature handling and a plane decomposed convolution to better distill representations from distorted features.
**iii)** Comprehensive validation of our methodologies on OpenOccupancy, with PVP showcasing significant performance improvements over contemporary techniques across both geometric and semantic metrics, emphasizing its utility for both lidar and multi-modality inputs.

---

I've made various edits for clarity, flow, and grammar while ensuring the technical essence remains intact. Always review changes to ensure they match the intended message and technical accuracy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The "Related Work" section you've provided is well-structured, giving a clear picture of the existing literature in the field of 3D occupancy prediction. I've made some edits for grammar, clarity, and coherence:

---

\paragraph{3D Occupancy Prediction.}
Historical tasks such as LiDAR segmentation or object detection typically predict labels for sparse LiDAR points or foreground objects. These endeavors often overlook the comprehensive representation of the surrounding environment and display limited adaptability to objects with atypical shapes. In contrast, 3D occupancy prediction~\cite{wang2023openoccupancy, behley2019semantickitti} aspires to assign a semantic label to every voxel within the perceptual range, positioning it as a fundamental aspect of 3D scene understanding in autonomous driving. Given the dense prediction space and cubic voxel labeling, most contemporary works~\cite{li2022bevformer,wei2023surroundocc, roldão2020lmscnet, yan2020sparse, li2020anisotropic} favor a Cartesian-based voxel model. Although they yield satisfactory results, these methods often sideline the polar-based representation. The appeal of this representation lies in its innate alignment with the non-uniform distribution of geometric and semantic data present in point clouds and camera outputs.

\vspace{-2mm}
\paragraph{Polar-based 3D object perception.}
The potential of polar or polar-like coordinate systems has been thoroughly assessed in previous undertakings. Both PolarNet~\cite{zhang2020polarnet} and Cylinder3D~\cite{zhu2021cylindrical} utilize polar-shaped partitions to evenly distribute points across grid cells during LiDAR segmentation. PolarStream~\cite{chen2021polarstream} extends the use of polar representation to 3D detection, introducing a polar-to-Cartesian sampling module and a range-stratified convolution. Moreover, PARTNER~\cite{nie2023partner} weaves in both long-range and localized attention for 3D detection, aiming to optimize the alignment of polar features. Notably, these methods don't grapple with the intricacies stemming from dense voxel prediction. This form of 3D representation accentuates distortion problems, particularly when juxtaposed against BEV or sparse 3D representations in feature propagation. To navigate these complications, our approach leans on the attention mechanism and decomposed convolution, addressing the visual distortion challenges inherent to polar coordinates.

\vspace{-2mm}
\paragraph{Transformer.}
The transformer's efficacy is well-established across various computer vision tasks. Building on the foundation laid by ViT~\cite{dosovitskiy2020image}, there has been an upsurge in the exploration of attention mechanisms. For instance, the Swin Transformer~\cite{swin} offers local window attention coupled with window shifting, while FAN~\cite{fan} emphasizes channel-wise global attention tailored for the nascent visual groups of transformers. Recently, there has been a surge in the adoption of transformer-based architectures in LiDAR-driven 3D object detection. Some studies~\cite{votr, fan2022embracing, he2022voxset} incorporate transformers as 3D backbones applied to sparse voxels, while others~\cite{nie2023partner, li2022bevformer} leverage transformers on BEV maps to extract global information and realign features. Contrasting these methodologies, our PVP is intentionally crafted, bearing in mind the nuances of the 3D tensor-based polar representation, to ameliorate the feature distortion challenge by honing in on effective representation.

---

Your content is dense with information, so always ensure that any modifications accurately represent your intended meaning and retain technical correctness.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}

Your method section introduction is concise and relatively clear. I've made minor edits to enhance the grammar and readability:

---

In this section, we introduce our \textbf{P}olar \textbf{V}oxel Occupancy \textbf{P}redictor (PVP) – a dense voxel prediction model tailored for polar BEV representation. We begin with an overview of the entire architecture in Sec.~\ref{Overall Architecture}. Subsequently, we delve into two pivotal contributions of PVP: the global representation propagation module (GRP Module) discussed in Sec.~\ref{grpmodule}, and the plane decomposed convolution (PD-Conv) elaborated in Sec.~\ref{pdconv}.

---

Remember to ensure that the references (like \ref{Overall Architecture}) match the exact labels used in your document, as I can't verify them here.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Your method section 2 is informative, but there are some grammatical and clarity issues. I'll go through and make corrections:

---

\subsection{Overall Architecture} \label{Overall Architecture}

For every 3D scene, our PVP model accepts a point cloud comprised of \(N_p\) points and several images capturing the surrounding environment. Each LiDAR point is characterized by a vector of point features \((r_p, \theta_p, x_p, y_p, z_p, i_p)\). Here, \((x_p, y_p, z_p)\) denotes the Cartesian coordinates, \((r_p, \theta_p)\) symbolizes the polar coordinates, and \(i_p\) represents the reflection intensity.

Our proposed \textit{PVP} is structured into five distinct parts:

1. \textit{Grid-based Backbones}: PVP includes two grid-based backbones. The 3D voxel-based backbone captures grid feature embeddings from points situated in voxels or pillars, transforming sparse point features into a dense 3D feature tensor aligned with polar coordinates. In parallel, a 2D image backbone extracts semantic features, subsequently projected into 3D spaces to enhance semantic performance.

2. \textit{Image-to-3D Encoder}: To fully harness the semantic features derived from images, contemporary studies~\cite{li2022bevformer, philion2020lift} have advocated for the elevation of features from image to 3D space via spatial projection. In our approach, we seamlessly integrate LSS~\cite{philion2020lift} for this purpose.

3. \textit{GRP Module}: This module ingests the sparse 3D tensor generated by both the 3D backbone and the Image-to-3D Encoder. It then outputs a dense 3D tensor by leveraging attention mechanisms for global feature propagation.

4. \textit{FPN Backbone}: This component processes the dense features, aggregating them for further use.

5. \textit{Polar Prediction Head}: This module transforms the polar-oriented 3D tensor into Cartesian voxel output.

---

Do ensure that the citations (like \cite{li2022bevformer}) match their intended references accurately, as I cannot verify them here.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The section you provided is quite technical, but I've tried to ensure clarity and correctness in terms of grammar. Here's the revised version of Method Section 3:

---

\subsection{Global Representation Propagation} \label{grpmodule}

In this section, we present the Global Representation Propagation module, an uncomplicated yet efficacious module that employs attention to selectively focus on crucial representative features for global alignment. The rationale behind this design stems from two observations: (1) the spatial resolution of polar grids fluctuates with the range, and (2) both the input 3D tensors exhibit sparsity. Given these factors, structural entities like roads, sidewalks, trees, or large edifices might face significant voids, accompanied by intense distortions in their occupied regions. These challenges contribute to an evident decline in performance for certain classes and negatively impact the efficacy of CNN-based predictors, particularly regarding their geometric performance given the dominant presence of these classes.

To mitigate these issues, our global representation re-alignment integrates two attention sub-modules: local cross-attention, which condenses multi-modal local features, and global decomposed attention, which ensures long-range feature propagation and re-alignment. We elucidate these sub-modules in the subsequent sections.

\vspace{-2mm}
\paragraph{Local Cross Attention} 

The proposed local cross attention takes the 3D feature \(F_p, F_i \in \mathbb{R}^{R \times A \times Z \times C}\) from both the 3D backbone and the image encoder. Here, \(R\), \(A\), and \(Z\) specify the resolutions of radial, azimuth, and height spaces, respectively, while \(C\) denotes the number of feature channels. An initial fused feature, \(F_{f}\), is derived using a 3D convolution as depicted:
\begin{equation} \label{3.2.1}
    F_{f} = Conv(Cat([F_p, F_i])).
\end{equation}
Aiming to cherry-pick representative features—thus reducing the computational demands of subsequent processes—we incorporate a local window-based max-selection operation. This involves segmenting \(F_{f}\) into non-overlapping windows sized \(W_g \times W_g \times W_g\). Denoting \(F_{f}[i]\) as the \(i\)-th local window, its representative feature, \(f_i\), is determined as:
\begin{equation} \label{3.2.2}
    f_{i} = \mathop{maxsel}(F_{f}[i]),
\end{equation}
where \(\mathop{maxsel}\) stands for a max selection operation that singles out the local-maxima within the local window \(f_i\). This suppression retains only the most pivotal features from each window, resulting in a compact global scene representation.

Each window's representative features are then compressed. Within this context, \(f_{i}\) and \(F_{f}[i]\) are the query and attending features of the \(i\)-th window, while \(p_{i}\) and \(p^{'}_{i}\) are the corresponding real pixel center coordinates in both polar and Cartesian systems. The dot-product attention for the \(i\)-th window is:
\begin{equation} 
    \begin{split}
        & Q_{i} = f_{i}W_{q}, K_{i} = F_{f}[i]W_{k}, V_{i} = F_{f}[i]W_{v}, \\
        & f^{rep}_{i} = softmax\left(\frac{Q_{i}K_{i}}{\sqrt{d}} \cdot V_{i}+E(p)\right),
    \end{split}
    \label{3.2.3}
\end{equation}
where \(W_{q}\), \(W_{k}\), and \(W_{v}\) represent the linear projections of query, key, and value. The function \(E(p)\) computes the relative positional encoding as:
\begin{equation} \label{3.2.4}
    E(p) = ReLU((p_i - p^{'}_{i}) \cdot W_{pos}).
\end{equation}
This cross-attention mechanism is applied to every column, resulting in a condensed feature map, \(F^{rep}\), for the subsequent global attention phase.

\vspace{-2mm}
\paragraph{Global Decomposed Attention} 

Employing the compressed representative features from the local cross attention, the global decomposed attention mechanism utilizes long-range self-attention for global feature propagation and re-alignment. This approach is motivated by the realization that particular classes often span across the entire scene, and different parts of a structural entity may exhibit varying distortion degrees. Such insights underscore the need for global spatial attention, enabling distant features to access nearby features for alignment without significant computational overhead. This ensures that features with similar radial, azimuth, or height dimensions possess a robust correspondence.

Given this premise, we integrate decomposed axis window attention to facilitate efficient global attention without compromising spatial structural information. Taking the radial axis as an exemplar, the compressed feature map, \(F^{rep}\), is partitioned into non-overlapping windows or strips along the radial axis. For a feature \(F_{rep}[i]\) in the \(i\)-th window, self-attention is employed as described by Eq.~\ref{3.2.3} and Eq.~\ref{3.2.4}. Our model leverages three stacked modules for information exchange. The second and third angular attentions use window partitions along the azimuth and height axes, respectively.

Following the global decomposed attention, the module invokes reverse local cross attention to disseminate representative features to every window within the feature map. Here, \(f_{i}\) and \(f^{'}_{i}\) are the query and attending features, respectively. The cross-attention formulation aligns with Eq.~\ref{3.2.3} and Eq.~\ref{3.2.4}.

---

Do note that you had two equations labeled as \(\ref{3.2.1}\). I've changed the second one to \(\ref{3.2.2}\) for clarity. Ensure that all equations and references align properly in your document.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The paper section provided is quite technical, related to machine learning, and its core concepts seem to be correct. I'll address the grammatical and stylistic aspects:

1. **Clarity**:
   - The first mention of "BEV" should be explained, such as "Bird's Eye View (BEV)" before using the acronym.
   
2. **Consistency**:
   - There's an inconsistency in using periods at the end of equation descriptions. For example, `\end{equation}` sometimes follows a period and sometimes doesn't. This should be consistent throughout.

3. **Grammar and Stylistic Fixes**:
   - "Detailedly" is not standard English. Consider replacing it with "In detail" or simply "Specifically".
   - "Both of the two issues" can be shortened to "Both issues".
   - "The output of the module $G = Cat([H, D])$ could be regarded as instance-wise geometric clues, which are supposed to help solve the occupation difference and the feature blurring issue." - The phrase "occupation difference" isn't clear in this context.
   - "For simplicity, the design of the task heads follows \cite{yin2020center}." - The word "follows" might be replaced with "is based on" or "is inspired by" for clarity.
   - "... which is also supervised in a smooth L1 loss." - Consider using "by" instead of "in" for clarity: "... which is also supervised by a smooth L1 loss."

4. **Spacing and Formatting**:
   - Ensure that there's a consistent space between paragraphs and subsections.
   - Ensure consistent usage of "~" for references like in "Sec.~\ref{1}".

5. **Additional Suggestions**:
   - Consider using a table or list format for the coefficients at the end for better clarity. For example:
     ```
     where the coefficients that balance the losses are set as:
     Waymo models: \( w_{reg} = 2, w_{fg} = 1, w_{dis} = 0.75, w_{iou} = 2 \)
     ONCE models: \( w_{reg} = 0.75, w_{fg} = 1, w_{dis} = 0.75, w_{iou} = 2 \)
     ```

6. **Referencing**:
   - Make sure all the references like `\cite{Lin_2017_ICCV}`, `\cite{yin2020center}`, etc. are properly cited in the bibliography or references section.

Lastly, if you have figures or tables, make sure they're properly labeled, captioned, and referenced in the text. Overall, the section seems well-structured, but these changes might make it more polished.

Certainly! I've made the suggested corrections and revisions to the provided section:

---

\subsection{Geometry-aware adaptive head} \label{pdconv}

In this section, we first investigate the potential drawbacks of polar detection heads. As discussed in Sec.~\ref{1}, the spatial resolution of polar grids varies depending on the range. This leads to two major challenges for the detection head: 

1) Feature blurring: Distant scenes are represented with low resolution, causing distant objects close to each other to become indistinguishable.
2) Shape variation: Traditional CNN-based regression heads often fail due to the varied distorted appearances of objects across different ranges or with different heading angles.

Both issues lead to regression difficulties in polar detectors.

To address these challenges, we introduce the Geometry-aware Adaptive (GA) head. This detection head differentiates features from different instances and explicitly integrates both instance information and geometric clues into the feature aggregation process. Below, we elaborate on the geometry-aware prediction module, detail the geometry-aware adaptive head, and finally present the task heads and total losses.

\vspace{-4mm}

\paragraph{Geometry-aware prediction.} To achieve fine-grained instance and geometric information, we utilize auxiliary supervisions with two prediction branches: a foreground segmentation branch and a regression branch. Specifically, both branches accept the Bird's Eye View (BEV) features, denoted as \( F^{neck} \), produced by the 2D backbone as input. The segmentation branch yields a heatmap \( H \in \mathbb{R}^{R \times A} \). Let \( \hat{H} \in \mathbb{R}^{R \times A} \) represent the corresponding target map of \( H \) and \( B_{bev} \in \mathbb{R}^{M \times 5} \) represent the BEV bounding boxes \( (x, y, w, h, \theta) \) of the ground-truth objects.

[...equations remain unchanged...]

The output of the module, given as \( G = Cat([H, D]) \), serves as instance-wise geometric clues. These clues are intended to address the occupation difference and the feature blurring issue. However, we observed that the auxiliary supervision alone doesn't boost the performance for polar detectors. To mitigate this, we further introduce a geometry-aware aggregation module to effectively harness the predicted information.

\vspace{-3mm}

\paragraph{Geometry-aware aggregation.} This sub-module harnesses the self-attention mechanism, supplementing it with positional priors of pixels in global coordinates and the predicted instance-wise geometric data. The module takes in the BEV map \( F^{neck} \) and the output \( G \) from the geometry-aware prediction module. We initially compute the geometry-aware embedding map \( F^{geo} \) from the geometric clues \( G \) and the real-world positional clues \( P \in \mathbb{R}^{R \times A \times 4} \).

[...equations remain unchanged...]

Employing the geometry-informed self-attention, the proposed module efficiently integrates instance and geometric insights into the feature aggregation and learning process. This produces features endowed with rich prior information for the succeeding detection heads.

\vspace{-2mm}

\paragraph{Task heads and losses.} To streamline our explanation, our design of the task heads is based on \cite{yin2020center}. We employ the matching-based assignment described in \cite{3dman} for target assignment. The predicted box parameters are optimized using the Smooth-$l_1$ loss, and the focal loss is applied to supervise the classification score. Additionally, inspired by RangeDet~\cite{fan2021rangedet}, we integrate an IoU regression head to predict the IoU between the bounding box and the best-matched ground truth annotations, supervised by a smooth L1 loss. During evaluation, the predicted confidence scores are reconciled with regression results as \( score' = score \times iou^{\alpha} \).

The overall loss for the proposed head is given by:

\begin{equation}
\small
    \mathcal{L} = \mathcal{L}_{cls} + w_{reg}\mathcal{L}_{reg} + w_{fg}\mathcal{L}_{fg} + w_{dis}\mathcal{L}_{dis} + w_{iou}\mathcal{L}_{iou},
\end{equation}

The coefficients that balance the losses are defined as:

For Waymo models: \( w_{reg} = 2, w_{fg} = 1, w_{dis} = 0.75, w_{iou} = 2 \)

For ONCE models: \( w_{reg} = 0.75, w_{fg} = 1, w_{dis} = 0.75, w_{iou} = 2 \)

---

Make sure to integrate this section appropriately with your paper, and ensure that all the citations link correctly to your bibliography or references section.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The text you provided is highly technical, so I'll be focusing mainly on grammar, punctuation, style, and consistency rather than the technical content itself. Here's a revision of your "Experiments" section:

---

\section{Experiments} 

We evaluate our method on the OpenOccupancy~\cite{wang2023openoccupancy} benchmark for 3D semantic occupancy prediction. In Sec.~\ref{sec_exp_setup}, we detail the datasets and implementation. We compare our method to other state-of-the-art methods in Sec.~\ref{sec_exp_open_occ}. Finally, we conduct ablation studies to investigate the effects of different components and designs of our method in Sec.~\ref{sec_abl}.

\subsection{Experimental setup}
\label{sec_exp_setup}

\noindent\textbf{OpenOccupancy dataset.} The newly introduced OpenOccupancy dataset~\cite{wang2023openoccupancy} is based on the data from the nuScenes dataset~\cite{caesar2020nuscenes}. It comprises 700 point cloud sequences for training and 150 sequences for validation. Each sequence lasts approximately 20 seconds with a Lidar frequency of 20Hz. There are 28,130 annotated frames for training and 6,019 for validation. Data collection involved a 32-lane Lidar and six surrounding cameras. The dataset has annotations for 16 classes and an additional free label to indicate unoccupied voxels. The primary metrics for 3D occupancy prediction are the Intersection of Union (IoU) – a geometric metric – and the mean IoU (mIoU) for all classes – a semantic metric. The evaluation range of OpenOccupancy is set from [-51.2m, -51.2m, -5m] to [51.2m, 51.2m, 3m] for the $X$, $Y$, and $Z$ axes, with a voxel resolution of [0.2m, 0.2m, 0.2m]. This results in an output volume of $512\times512\times40$ for occupancy prediction. For our model on the OpenOccupancy dataset, the perception range is [0.3m, 73.0m] for the $\rho$ axis, [$-\pi$, $\pi$] for the $\phi$ axis, and [-5m, 3m] for the \textit{z} axis.

\subsection{Implementation Details}

\noindent\textbf{Model Architecture.} For a fair comparison, we utilize the same pipeline as CONet~\cite{wang2023openoccupancy}, including its training scheme and head design. For voxelization, we transform the original point cloud into a sparse volume of dimensions $(H, W, D)=(1024, 1344, 80)$, where each dimension represents the $\rho$, $\phi$, and \textit{z}, respectively. In the Lidar backbone, we maintain the CONet backbone but substitute the basic block with our proposed spatially decomposed convolution block. The final volume representation from this pipeline has dimensions $(\mathcal{H}, \mathcal{W}, \mathcal{D}) = (128, 168, 10)$, which is an 8x down-sampling from the initial volume.

\noindent\textbf{Optimization.} During training, we employ the Adam optimizer with a weight decay of 0.01 and a cosine learning rate scheduler with a maximum value of 3e-4. We also use a linear warm-up for the first 500 iterations. For occupancy prediction, we follow OpenOccupancy~\cite{wang2023openoccupancy} and include an affinity loss to optimize both geometric and semantic metrics. Our models are trained over 25 epochs using a batch size of 8 across 8 V100 GPUs. Owing to resource constraints, the results of our ablation studies are reported based on models trained for five epochs.

[... Remainder of the text seems to be in good shape ...]

---

I've streamlined some sentences, ensured consistency in style, and made minor grammar corrections. Make sure that my edits maintain the intended technical meaning, and always double-check citations and cross-references to ensure they're correct and functional.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Your conclusion section is concise and clear. I'll make some small grammar and style adjustments:

---

\section{Conclusions}

In this work, we revisited the challenges of feature distortion and feature propagation in the polar representation of 3D space, which severely restrict the efficacy of polar-based 3D occupancy predictors. To address these challenges, we introduced PVP, an efficient 3D occupancy predictor in the polar coordinate system. PVP mitigates feature distortion using spatially decomposed convolution and enhances feature propagation by employing a long-range attention mechanism through our proposed GRP module. Our results show that the proposed method significantly outperforms previous polar-based methods and delivers competitive performance when compared to state-of-the-art methods. We hope our work will inspire further research in polar-based 3D perception.

---

I've refined the text for improved flow and clarity. Always ensure that my edits accurately capture the technical nuances of your work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Review 1:

Of course! I'll provide a review comment for the provided sections of your conference paper:

---

**Review Comment on "Title Not Provided" by [Author Name(s) Not Provided]**

**General Feedback:**
This paper addresses an important topic in the realm of 3D space representation and proposes a novel method, PVP, to overcome inherent challenges with polar-based 3D occupancy predictors. The work is clear, methodologically sound, and well-organized. However, there are areas that could benefit from clarification and refinement.

**Strengths:**

1. **Relevance of the Problem:** The paper tackles the significant challenge of feature distortion and propagation in polar representations, which is pertinent for many applications in computer vision and robotics.
  
2. **Technical Depth:** The introduction of PVP and its components, like the spatially decomposed convolution and the GRP module, showcases the depth of the research. The innovative approach to enhance feature propagation is commendable.

3. **Clear Structure:** The paper follows a logical flow, moving from the problem definition to the introduction of the solution, followed by experimental evaluations.

**Areas of Improvement:**

1. **Motivation & Background:** While the paper does touch upon the challenges of the polar representation, it might benefit from a more comprehensive literature review, setting the context and drawing contrasts with existing solutions.

2. **Clarifications on Methodology:** The section on 'Implementation Details' could be expanded to provide readers with a deeper understanding of the choices made, especially concerning the GRP module and the spatial decomposed convolution block. 

3. **Results Discussion:** While the results seem promising, it would be beneficial to have a more detailed discussion on the implications of these results. For instance, what does the significant performance gain signify in real-world applications? Are there specific scenarios where PVP might not be the best choice?

4. **Grammar & Style:** The paper would benefit from a thorough proofreading to fix minor grammatical errors and improve sentence structures for clarity and conciseness.

**Conclusion:**
Overall, the paper provides a solid contribution to the field. With some refinements and expansions on the methodology and results discussion, it has the potential to be a significant reference for future research in polar-based 3D perception. I look forward to seeing the revisions and the final version of the work.

---

Note: Always ensure that the review is in line with the standards and expectations of the conference or journal where the paper is being submitted.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
can you give me a review comment on this paper writing? from the viewpoint of a fresh researcher, to tell which part is hard to understand.
Review :

Of course! Reviewing the provided text from the perspective of a fresh researcher, here are some comments:

---

**General Comment:** The paper seems to discuss advanced topics in the domain of 3D occupancy prediction using polar representations. Given the complexity of the subject matter, it's expected that a fresh researcher may need supplementary materials or prior foundational knowledge to grasp the content fully.

1. **Introduction to the Problem:** 
   - Comment: While the problem is stated, a clearer introductory foundation on why the polar representation is crucial, and its typical applications, would be beneficial for a newcomer to the field.

2. **Terminologies and Concepts:** 
   - Comment: Terms such as "polar representation," "3D occupancy predictor," "spatial decomposed convolution," and "long-range attention mechanism" could be jargon for someone unfamiliar with the domain. A brief definition or elaboration when these terms first appear would be helpful.
  
3. **Dataset and Implementation Details:** 
   - Comment: The section dives into details about the datasets used, including specifics about the OpenOccupancy dataset. While this is essential for replication and understanding the experiments, some contextual background about why certain choices were made might be useful. For instance, why was the OpenOccupancy dataset chosen over others?
   - The information about the dimensions and axes might be challenging for someone not familiar with 3D data representation. Visualization or a brief overview might help.

4. **Model Architecture and Optimization:** 
   - Comment: While the paper delves into the specifics of the model architecture and optimization techniques, a high-level overview or visualization of the model's flow and components could assist in understanding the paper's core contributions.

5. **Results and Comparisons:** 
   - Comment: It's great to see that the model outperforms previous methods. However, for someone new, understanding the importance of the metrics used (like mIoU and IoU) would be valuable. Why are these metrics crucial, and what do they signify?

6. **Ablation Studies:** 
   - Comment: This section is dense with technical details. Breaking down the significance of each component, what they bring to the model, and why certain modules were chosen or disregarded would be beneficial. Visual aids or simplified explanations can assist in making this section more accessible.

7. **Conclusion:** 
   - Comment: The conclusion provides a succinct recap of the paper's main points. However, adding a line or two about the potential real-world applications or implications of this work could provide context to newcomers about the importance of this research.

---

Overall, while the paper seems technically sound and detailed, incorporating visual aids, clearer explanations of terminologies, and some context on the choices made would make it more comprehensible for fresh researchers or those outside the immediate domain.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

